Approximating Knapsack and Partition via Dense Subset Sums

Knapsack and Partition are two important additive problems whose fine-grained complexities in the $(1-\varepsilon)$-approximation setting are not yet settled. In this work, we make progress on both problems by giving improved algorithms. - Knapsack can be $(1 - \varepsilon)$-approximated in $\tilde O(n + (1/\varepsilon) ^ {2.2} )$ time, improving the previous $\tilde O(n + (1/\varepsilon) ^ {2.25} )$ by Jin (ICALP'19). There is a known conditional lower bound of $(n+\varepsilon)^{2-o(1)}$ based on $(\min,+)$-convolution hypothesis. - Partition can be $(1 - \varepsilon)$-approximated in $\tilde O(n + (1/\varepsilon) ^ {1.25} )$ time, improving the previous $\tilde O(n + (1/\varepsilon) ^ {1.5} )$ by Bringmann and Nakos (SODA'21). There is a known conditional lower bound of $(1/\varepsilon)^{1-o(1)}$ based on Strong Exponential Time Hypothesis. Both of our new algorithms apply the additive combinatorial results on dense subset sums by Galil and Margalit (SICOMP'91), Bringmann and Wellnitz (SODA'21). Such techniques have not been explored in the context of Knapsack prior to our work. In addition, we design several new methods to speed up the divide-and-conquer steps which naturally arise in solving additive problems.

==> determi.tex <==
\label{sec:determi}


\subsection{For small $n$} \label{sec:small}

\begin{lemma}
\label{lem:dc}
For parameters $c,m\in N^+$, and multiset $X\subseteq \N^+ \cap [m,2m]$ of size $|X|=n$, one can compute $\caSC^{c}(X)$ in $\tilde O(c^2 (n+m))$ time deterministically.
\end{lemma}

\begin{proof}
We use densified divide and conquer.
    
    
    blablabla\cnote{}
    
     we first sort numbers in increasing order of $k$ and then try to bound the running time using similar density argument as seen in the algorithm for partition.
     
     \begin{algorithm2e}
	Given $x_1<\dots<x_{|X|}$, the sorted list of elements of $X$ \\
	\caption{blabla}
	\label{algo:dc}
\end{algorithm2e}
     

The algorithm itself is similar: if we are merging two intervals $[l, mid]$ and $[mid, r]$, for all pairs $(z, x)$ (denoting number $z \times k + x \times b$, as in Koiliaris and Xu's algorithm) in the sumset, we let $y = z - xl$ (so $z = x \times l + y$). We can do 2D-FFT on $(x, y)$. Suppose $m = t / n ^ u$. Suppose we are on the layer where the number of numbers in the intervals are $s = O(n ^ v)$. Let $\tau = \min(s, t / m) = n ^ {\min(u, v)}$. The transition runs in $\tilde O(\tau ^ 2 \times (r - l))$ time.
\end{proof}


\begin{cor}
For parameters $m,t\in N^+, m\le t$, and multiset $X\subseteq \N^+ \cap [m,2m]$ of size $|X|=n$, one can compute $\caSC(X;t)$ in  time deterministically.
\end{cor}
\begin{proof}
\end{proof}

\begin{theorem} \label{theorem:small}
   Given multiset $X \subseteq \N^+$ of size $|X|=n$, there is a deterministic algorithm that computes $\caS(X;t)$ in $\tilde O(n ^ {1 / 3}t)$ time.
\end{theorem}

\begin{proof}x
First apply \cref{lem:multiset}.

Let $p = \Theta(n ^ {1 / 3})$ and express each number $u$ inside the group as $u = kp + b$. We computer answers for each $b$ and they can be merged in $\tilde O(pt) = \tilde O(n ^ {1 / 3}t)$ time.
\end{proof}

First, divide numbers into $O(\log{t})$ groups, each containing numbers in some interval $[m, 2m]$. The answers can be merged in $\tilde O(t)$ time. Consider computing the answer for each group.

Pick $c = \lfloor t/m\rfloor $ as upper bound on cardinality.   For each $b\in \F_p$, apply \cref{lem:dc} to the reduced items, compute $\caSC^c$ 


For each $b$, we build on Koiliaris and Xu's method, but

Alternatively, we can simply ignore $p$ and do 1D-FFT on the sumsets. This runs in $\tilde O(m \time \tau)$ time per transition.

If we do 2D-FFT, the running time for the entire layer is
\begin{align*}
    \tilde O(\tau ^ 2 \times m / p) = \tilde O(n ^ {2\min(u, v) - u - 1 / 3}t).
\end{align*}

If we do 1D-FFT, the running time for the entire layer is
\begin{align*}
    \tilde O(m \time \tau \times n / s) &= \tilde O(t n ^ {\min(u, v) + 1 - u - v})) \\
    &= \tilde O(t n ^ {1 - \max(u, v)}).
\end{align*}

So the running time is at most
\begin{align*}
    \tilde O(n ^ {\min(2\min(u, v) - u - 1 / 3, 1 - \max(u, v))}t).
\end{align*}

Obviously this is maximum when $v = u$, so the running time becomes
\begin{align*}
    \tilde O(n ^ {\min(u - 1 / 3, 1 - u)}t),
\end{align*}
which takes the maximum of $\tilde O(n ^ {1 / 3}t)$ when $u = 2 / 3$.

This proves Lemma \ref{lemma:small}.

\subsection{For large $n$}

\begin{theorem} \label{theorem:large}
   Given multiset $X \subseteq \N^+$ of size $|X|=n$, there is a deterministic algorithm that computes $\caS(X;t)$ in  $\tilde O(n + t ^ {8 / 7})$ time.
\end{theorem}



We can easily convert the multset into a set with only logarithmic overhead.

Let be $n$ is the size of the set of the group of numbers between $[m, 2m]$. Let $m = t / n ^ u$.

Recall Theorem \ref{theo:galil}, for every $m$, for every $t ^ {\prime} \gg m ^ 2 / n$, that is $t ^ {\prime} \gg t ^ 2 / n ^ {2u + 1}$, then we decide whehter $t ^ {\prime}$ is in the sumset in constant time. This part contributes $O(t)$ time in total and will not be the bottleneck. After that we perform the algorithm in section \ref{sec:small} for every $t ^ {\prime} = \Theta(t ^ 2 / n ^ {2u + 1})$. 

Analysis:

The running time is at most
\begin{align*}
    \tilde O(t + n ^ {\min(u - 1 / 3, 1 - u)}t ^ {\prime}) &= \tilde O(n ^ {\min(u - 1 / 3, 1 - u)}t ^ 2 / n ^ {2u + 1})
    &= \tilde O(t + n ^ {\min(-u - 4 / 3, -3u)}t ^ 2)
\end{align*}

Let $n = t ^ w$. Note that we can choose the better one between the algorithm here and the algorithm in section \ref{sec:small}, so the running time is
\begin{align*}
    \tilde O(\min(t + {t ^ w} ^ {\min(-u - 4 / 3, -3u)}t ^ 2, {t ^ w} ^ {\min(u - 1 / 3, 1 - u)}t)),
\end{align*}
which is
\begin{align*}
    \tilde O(t ^ {\max(1, \min(2 - w\max(u + 4 / 3, 3u), 1 + w\min(u - 1 / 3, 1 - u)))}).
\end{align*}
Which takes a maximum of $\tilde O(t ^ {8 / 7})$ when $w = 3 / 7$ and $u = 2 / 3$. \xnote{I wrote some Python code to compute this numerically. Should be correct.}

This proves Lemma \ref{lemma:large}.

\xnote{In the final write-up can make this a 2-phase algorithm with 2D-FFT as the bottom phase (where the parameter $p$ comes into play) and 1D-FFT as the top phase.}

